Faro: A framework for measuring the scientific performance of petascale Rubin Observatory data products

The Vera C. Rubin Observatory will advance many areas of astronomy over the next decade with its unique wide-fast-deep multi-color imaging survey, the Legacy Survey of Space and Time (LSST). The LSST will produce approximately 20TB of raw data per night, which will be automatically processed by the LSST Science Pipelines to generate science-ready data products -- processed images, catalogs and alerts. To ensure that these data products enable transformative science with LSST, stringent requirements have been placed on their quality and scientific fidelity, for example on image quality and depth, astrometric and photometric performance, and object recovery completeness. In this paper we introduce faro, a framework for automatically and efficiently computing scientific performance metrics on the LSST data products for units of data of varying granularity, ranging from single-detector to full-survey summary statistics. By measuring and monitoring metrics, we are able to evaluate trends in algorithmic performance and conduct regression testing during development, compare the performance of one algorithm against another, and verify that the LSST data products will meet performance requirements by comparing to specifications. We present initial results using faro to characterize the performance of the data products produced on simulated and precursor data sets, and discuss plans to use faro to verify the performance of the LSST commissioning data products.

==> Makefile <==
DOCTYPE = DMTN
DOCNUMBER = 211
DOCNAME = $(DOCTYPE)-$(DOCNUMBER)

tex = $(filter-out $(wildcard *acronyms.tex) , $(wildcard *.tex))

GITVERSION := $(shell git log -1 --date=short --pretty=%h)
GITDATE := $(shell git log -1 --date=short --pretty=%ad)
GITSTATUS := $(shell git status --porcelain)
ifneq "$(GITSTATUS)" ""
	GITDIRTY = -dirty
endif

export TEXMFHOME ?= lsst-texmf/texmf

$(DOCNAME).pdf: $(tex) meta.tex local.bib  acronyms.tex authors.tex
	latexmk -bibtex -xelatex -f $(DOCNAME)

# Acronym tool allows for selection of acronyms based on tags - you may want more than DM
acronyms.tex: $(tex) myacronyms.txt
	$(TEXMFHOME)/../bin/generateAcronyms.py -t "DM" $(tex)

authors.tex:  authors.yaml
	$(TEXMFHOME)/../bin/db2authors.py -m spie > authors.tex 


.PHONY: clean
clean:
	latexmk -c
	rm -f $(DOCNAME).{bbl,glsdefs,pdf,xdv}
	rm -f meta.tex

.FORCE:

meta.tex: Makefile .FORCE
	rm -f $@
	touch $@
	printf '%% GENERATED FILE -- edit this in the Makefile\n' >>$@
	printf '\\newcommand{\\lsstDocType}{$(DOCTYPE)}\n' >>$@
	printf '\\newcommand{\\lsstDocNum}{$(DOCNUMBER)}\n' >>$@
	printf '\\newcommand{\\vcsRevision}{$(GITVERSION)$(GITDIRTY)}\n' >>$@
	printf '\\newcommand{\\vcsDate}{$(GITDATE)}\n' >>$@


==> acronyms.tex <==
\addtocounter{table}{-1}
\begin{longtable}{p{0.145\textwidth}p{0.8\textwidth}}\hline
\textbf{Acronym} & \textbf{Description}  \\\hline

API & Application Programming Interface \\\hline
AST & NSF Division of Astronomical Sciences \\\hline
AURA & Association of Universities for Research in Astronomy \\\hline
CCD & Charge-Coupled Device \\\hline
CI & Continuous Integration \\\hline
DC2 & Data Challenge 2 (DESC) \\\hline
DE & dark energy \\\hline
DESC & Dark Energy Science Collaboration \\\hline
DMTN & DM Technical Note \\\hline
DP0 & Data Preview 0 \\\hline
DRP & Data Release Production \\\hline
FITS & Flexible Image Transport System \\\hline
FWHM & Full Width at Half-Maximum \\\hline
HSC & Hyper Suprime-Cam \\\hline
IDF & Interim Data Facility \\\hline
LPM & LSST Project Management (Document Handle) \\\hline
LSST & Legacy Survey of Space and Time (formerly Large Synoptic Survey Telescope) \\\hline
LSSTC & LSST Corporation \\\hline
PDR2 & Public Data Release 2 (HSC) \\\hline
PSF & Point Spread Function \\\hline
REST & REpresentational State Transfer \\\hline
RMS & Root-Mean-Square \\\hline
RSP & Rubin Science Platform \\\hline
RTN & Rubin Technical Note \\\hline
SLAC & SLAC National Accelerator Laboratory \\\hline
SPIE & The international society for optics and photonics \\\hline
SQR & SQuARE document handle \\\hline
SRD & LSST Science Requirements; LPM-17 \\\hline
UI & User Interface \\\hline
YAML & Yet Another Markup Language \\\hline
arcmin & arcminute minute of arc (unit of angle) \\\hline
\end{longtable}


==> summary.tex <==
% 100 word summary sunmitted to SPIE
 
\noindent \textbf{100 word summary} \newline
\noindent Once operational, up to 20TB of raw imaging data will be collected by Rubin Observatory's Legacy Survey of Space and Time (LSST) per night and processed by the LSST Science Pipelines to produce science-ready data products -- processed images, catalogs and alerts.  
To ensure that these data products enable transformative science with LSST, stringent requirements have been placed on their quality and scientific fidelity.
In this paper we introduce {\ttfamily faro}, a framework for automatically and efficiently computing scientific performance metrics on the LSST data products for units of data of varying granularity, ranging from single-detector to full-survey summary statistics. 

\end{abstract}


